PyTorchGeoNodes: Enabling Differentiable Shape Programs for 3D Shape Reconstruction

We propose PyTorchGeoNodes, a differentiable module for reconstructing 3D objects and their parameters from images using interpretable shape programs. Unlike traditional CAD model retrieval, shape programs allow reasoning about semantic parameters, editing, and a low memory footprint. Despite their potential, shape programs for 3D scene understanding have been largely overlooked. Our key contribution is enabling gradient-based optimization by parsing shape programs, or more precisely procedural models designed in Blender, into efficient PyTorch code. While there are many possible applications of our PyTochGeoNodes, we show that a combination of PyTorchGeoNodes with genetic algorithm is a method of choice to optimize both discrete and continuous shape program parameters for 3D reconstruction and understanding of 3D object parameters. Our modular framework can be further integrated with other reconstruction algorithms, and we demonstrate one such integration to enable procedural Gaussian splatting. Our experiments on the ScanNet dataset show that our method achieves accurate reconstructions while enabling, until now, unseen level of 3D scene understanding.

==> figs_latex/chair_code.tex <==
\begin{minipage}{0.55\textwidth}
\lstset{escapeinside={<@}{@>}}
\begin{lstlisting}[
    basicstyle=\ttfamily\footnotesize,
    backgroundcolor=\color{lightgray!20},
    frame=single,
    % keywordstyle=\color{blue}\bfseries,
    morekeywords={true, false},
    numberstyle=\tiny\color{gray},
    xleftmargin=10pt,
    xrightmargin=10pt,
    breaklines=true,
    showstringspaces=false
]
{<@\color{white}\colorbox{black}{\textbf{P}}@>Seat: { Width: 0.45,  Height: 0.55,  Depth: 0.44,  Thickness: 0.13}, <@\color{white}\colorbox{black}{\textbf{P}}@>Legs: {Legs Type: 'four-legged',  Size: 0.08, <@\color{white} \colorbox{black}{\textbf{P}}@>Support{ Has Leg Support: true,  Thickness: 0.04,  Offset-1: 0.21, <@\color{white}\colorbox{black}{\textbf{P}}@>{Offset-2: 0.32}}} <@\color{white}\colorbox{black}{\textbf{P}}@>Back: {Has Back: true, Height: 0.36, Thickness: 0.05,<@\color{white}\colorbox{black}{\textbf{P}}@>Backrest: { Backrest Scale: 0.7,  Backrest Offset Scale: 0.78,}}, Arms: {Has Arms: false}}
\end{lstlisting}
\end{minipage}


==> figs_latex/lim_fig.tex <==
\newcommand{\limresult}[2]{
\includegraphics[height=\niceresultheight]{figures/lim_results/#1_obj_#2/overlay.jpg} &
\includegraphics[height=\niceresultheight]{figures/lim_results/#1_obj_#2/rec_3d.png} \\
}


\begin{figure}[t]
    \vspace{-0.6cm}
    \centering
    \resizebox{1\textwidth}{!}{
    \scriptsize
    \begin{tabular}{cc}
        \limresult{scene0025_00}{2}
        \limresult{scene0046_01}{4}
        % \limresult{scene-1}{-1} \\[-0.3cm]
          \hspace{1.5cm} retrieved model \hspace{0.2cm} GT model & \hspace{-0.1cm} retrieved model \hspace{-0.1cm} GT model \\        
         % \includegraphics[height=1.5cm]{figures/qualitative_results/scene0435_00_obj_20/overlay.jpg} & 
         % \includegraphics[height=1.5cm]{figures/qualitative_results/scene0435_00_obj_20/rec_3d.png}\\
    \end{tabular}
    }
    % \includegraphics{}
    \vspace{-0.3cm}
    \caption{\textbf{Visualizations of current limitations.} First row: Even though our shape program considers legs, such details are usually very small, making the reconstruction very challenging especially given the noisy observations from the ScanNet dataset. The annotations from Scannotate have similar issues. Second row: Our Table shape program does not yet consider cabinets built into tables. }
    \label{fig:limfig}
\end{figure}

    % \caption{\sinisa{Overview of limitations of our approach. For each sample (a) an exemplary view, (b) overlay of our projected reconstructions into the input view, (c) overlay with Scannotate CAD model projections, (d) our 3d reconstruction, and (e) Scannotate reconstruction. As shown in the first example, even though our shape program allows modelling of leg arms, such details are usually very small, which makes the reconstruction very challenging especially given the noisy observations from the ScanNet dataset. We observe that manual annotations from Scannotate have similar issues. In the second example, we show a situation that we did not consider when designing our shape program for the table category as we are not able to model cabinets that are built into tables. Similarly in the third example, while we reconstruct the armrest, we do not model different configurations. We observe that model from the Scannotate dataset is reconstructed using the correct armrest, but the depth of the chair seat is too large in contrast. CAD model retrieval methods do not allow for the scaling of individual components. We note that in both the second and the third example, shape programs could be simply edited to also consider these scenarios.}}

==> preamble_1.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{graphicx} % For including images
\usepackage{multirow}
\usepackage{geometry}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{float}
\usepackage{enumitem}
\usepackage[dvipsnames]{xcolor}

\usepackage{cellspace}
